On Geometry of Coned-Off Spaces and Cannon-Thurston Maps

A typical question addressed in this paper is the following. Suppose $Z\subset Y\subset X$ are hyperbolic spaces where $Z$ is quasiconvex in both $Y$ and $X$. Let $\HAT{Y}$ and $\HAT{X}$ denote the spaces obtained from $Y$ and $X$ respectively by coning off $Z$ as defined by Farb. {\em If the inclusion of the coned-off spaces $\HAT{Y}\map \HAT{X}$ admits the Cannon-Thurston (CT) map then does the inclusion $Y\map X$ also admit the Cannon-Thurston map?} The main result of this paper answers this question affirmatively provided $\HAT{Y}\map \HAT{X}$ satisfies Mitra's criterion for the existence of CT maps, although the answer in general is negative. The main application of our theorem is in the context of acylindrical complexes of hyperbolic groups. A. Martin proved a combination theorem for developable, acylindrical complexes of hyperbolic groups. Suppose $(\mathcal G, \YY)$ is an acylindrical complex of hyperbolic groups with universal cover $B$ which satisfy the hypotheses of Martin's theorem. Suppose $\YY_1\subset \YY$ is a connected subcomplex such that the subcomplex of groups $(\mathcal G, \YY_1)$ also satisfies the hypotheses of Martin's theorem, it has universal cover $B_1$ and the natural homomorphism $\pi_1(\mathcal G, \YY_1)\map \pi_1(\mathcal G, \YY)$ is injective. It follows from the main theorem of this paper that the inclusion $\pi_1(\mathcal G, \YY_1)\map \pi_1(\mathcal G, \YY)$ admits the CT map if the inclusion $B_1\rightarrow B$ satisfies Mitra's criterion. Also $\pi_1(\mathcal G, \YY_1)$ is quasiconvex in $\pi_1(\mathcal G, \YY)$ if in addition $B_1$ is qi embedded in $B$.

==> part3-060423.tex <==

%\BLUE{Where is that short exact sequence example?}
\section{Consequences and examples}\label{section 4}
In this section we discuss several applications of the results of the previous section. We start with the following.

\subsection{Application to (relatively) hyperbolic groups}
Theorem \ref{electric ct} has the following immediate group theoretic consequences. 
Before stating the results we note that
in both the theorems mentioned below we have the following set-up. 

%\BLUE{please make a remark on local finiteness on subgroups of a groups somewhere.}
\begin{enumerate}
\item We have a group $G$ and a subgroup $H$ of $G$.

\item Moreover, there are subgroups $K_1, K_2,\cdots, K_n$ in $G$ and $K'_1,K'_2,\cdots, K'_m$ in $H$
such that the following hold:

(1*) {\em For all $1\leq i\leq m$ there is $g_i\in G$ and $1\leq r_i\leq n$ such that $K'_i= H\cap g_iK_{r_i}g^{-1}_i$.}

(2*)  {\em For all $g\in G$ and $1 \leq i\leq n$, there is $1\leq l\leq m$ and $h\in H$ such that 
$H\cap gK_i g^{-1}= hK'_lh^{-1}$.}

We note that for all $i, 1\leq i\leq m$ and all $h\in H$ we have $hK'_i\subset hg_iK_{r_i}g^{-1}_i$ by (1*). Thus if
$D=\max\{d(1,g_i): 1\leq i\leq m\}$ then $hK'_i\subset N_D(hg_i K_{r_i})$ for all $1\leq i\leq m$ and
$h\in H$ where the neighborhood is taken in a Cayley graph of $G$. 

\item {\em Let $\hat{H}$ be the coned-off space obtained from $H$ by coning the various cosets of $K'_i$'s 
and $\hat{G}$ be the coned-off space obtained from $G$ by coning off the cosets of the various $K_i$'s.} 

Let $\hat{\hat{G}}$ be the coned-off spaces obtained from $G$ by coning off the $D$-neighborhoods of the cosets of 
$K_i$'s in $G$. Then there are natural inclusion maps $\phi_1:\hat{H}\map \hat{\hat{G}}$ and $\phi_2:\hat{G}\map \hat{\hat{G}}$ respectively where the latter is a quasiisometry by Lemma \ref{basic cone-off 3}. 

\item {\em Let $\iota:H\map G$ denote the inclusion map and let  $\hat{\iota}:\hat{H}\map \hat{G}$ be the natural map
such that $\phi_2\circ \hat{\iota}=\phi_1$. }

We note that since $\phi_2$ is a quasiisometry, $\phi_1$ satisfies Mitra's criterion or admits the CT map- 
in case the coned-off spaces are hyperbolic, if and only if the same is true about $\hat{\iota}$.
 
\end{enumerate}


\begin{theorem}\label{application 1}
Suppose $H< G$ are hyperbolic groups, $K_1, K_2, \cdots, K_n$ are quasiconvex subgroups of $G$
and $K'_1, K'_2,\ldots, K'_m$ are subgroups of $H$ which are all quasiconvex in $G$ such that (1*) and (2*) hold.
Then assuming the notation in (3) and (4) we have the following:

(1) If the map $\hat{\iota}: \HAT{H}\map \HAT{G}$ satisfies Mitra's criterion then there is a CT map 
$\partial \iota: \partial H\map \partial G$. Moreover, if the CT map $\partial \hat{\iota}$ is injective then $H$ is quasiconvex in $G$.

(2) Conversely, suppose the CT map for the inclusion $\iota: H\map G$ exists. Then the CT map for 
$\hat{\iota}:\hat{H}\map \hat{G}$ exists if and only if for any coset $gK_i, 1\leq i\leq n$ and 
$\xi\in \Lambda(gK_i)$ either $\xi\not\in \partial i(\partial H)$
or there is $h\in H, 1\leq j\leq m$ such that $\xi\in \Lambda_G(h K'_j)$.
\end{theorem} 
\proof The first part of (1) is immediate from Theorem \ref{electric ct}. One notes that $K'_i$'s are quasiconvex
in $H$ as well by \cite[Lemma 2.2]{ilyakapovichcomb}. Also when the CT map $\partial H\map \partial G$ exists, 
it is injective if and only if so is the CT map
$\partial \HAT{H}\map \partial \HAT{G}$. Hence, the second part of (1) follows by Lemma \ref{inj of ct}.
% $H$ is quasiconvex in $G$. \qed
(2) is immediate from Proposition \ref{main converse}. \qed

%We shall see an application of the above theorem in the next subsection. 
For background on relatively hyperbolic groups, one is referred to some standard references like \cite{bowditch-relhyp},\cite{farb-relhyp}
\cite{groves-manning}, and \cite{hru-rel}. One is referred to \cite[Definition 6.2]{hru-rel} for the definition of
a relatively quasiconvex subgroup of a relatively hyperbolic group. Now as another application of Theorem \ref{electric ct} 
one has the following.

\begin{theorem}\label{application 2}
Suppose $H<G$ are finitely generated groups and $K_i<G$, $1\leq i\leq n$ and $K'_j<H$, $1\leq j\leq m$
such that that (1*), (2*) hold. Moreover suppose that $G$ is hyperbolic relative to $K_i$'s and $H$
is hyperbolic relative to $K'_j$'s. Then with the notation (3) and (4) we have the following:

If $\hat{\iota}:\HAT{H}\map \HAT{G}$ satisfies Mitra's criterion then the CT map exists in level of the Bowditch 
boundaries of the groups $\partial_B H\map \partial_B G$. Moreover, if the CT map is injective then 
$H$ is relatively quasiconvex in $G$.
\end{theorem}
{\bf Discussion.} Before we present a proof of the theorem let us first try to make sense of
the statement of the theorem.
\begin{enumerate}
\item By attaching attaching hyperbolic cusps to a Cayley graph of $G$ along the various cosets
of $K_i$'s we get a hyperbolic metric space, say $X'$; e.g. see \cite{groves-manning}. 
The {\em Bowditch boundary} (\cite{bowditch-relhyp}) of $G$ (with respect $\{K_i\}$) is defined 
to be $\partial_s X'$. It is a standard fact that $\partial_s X'$ independent on the choice of
Cayley graph of $G$. We shall denote it by $\partial_B G$. Since $X'$ is a proper hyperbolic metric space,
$\partial_B G$ is a compact metrizable space.
 
\item Let $D\geq 0$ be such that $K'_i\subset N_D(g_iK_{r_i})\cap H$ for all $1\leq i\leq m$.
After attaching hyperbolic cusps along the $D$-neighborhoods of all the cosets of the subgroups 
$\{K_i\}$ in a Cayley graph of $G$ we get a space, say $X$. Now, $X$ is also hyperbolic since 
$X$ is quasiisometric to $X'$. \RED{ref??}

\item Let $Y$ be the space obtained by attaching hyperbolic cusps to a Cayley graph of $H$ along 
the cosets of the subgroups in $\{K'_i\}$. The resulting space, say $Y$, is also hyperbolic.
Note that $\partial_B H=\partial_s Y$ and $Y\subset X$. 

\item When the CT map $\partial Y\map \partial X$ exists then we say that the inclusion $H\map G$ 
admits the CT map in the level of the Bowditch boundaries. Lastly it is clear that $H$ naturally 
acts on $Y$ isometrically and hence it induces an action on $\partial_B Y$. For a proof see 
\cite[Section 3]{groves-manning}. This action is geometrically finite by \cite[Theorem 5.4]{hru-rel}.
\end{enumerate}


{\em Proof of Theorem \ref{application 2}:} Suppose $\HAT{X}$ and $\HAT{Y}$ are the spaces
obtained from $X,Y$ respectively by coning off all the hyperbolic cusps in $X$ and $Y$ respectively. 
`We note that $\hat{G}$ is naturally quasiisometric to $\HAT{X}$. 
Thus the inclusion map $\HAT{Y}\map \HAT{X}$ satisfies Mitra's condition. It is a standard fact 
that the hyperbolic cusps are uniformly quasiconvex in the respective cusped spaces. \RED{ref??}
Hence, all the hypotheses of Theorem \ref{electric ct} checks out. It follows that
CT map exists for the inclusion $Y\map X$.

\RED{Precise references need, like Thm/Lemma/Prop numbers:}
For the second part we note that $\partial_B H$ is equivariantly homeomorphic to the image of the CT map,
since the Bowditch boundaries are compact, Hausdorff spaces as mentioned in the discussion above. 
Hence, $H$-action on the image of the CT map is geometrically finite. We note that the $H$-action on
$\partial_B H$ is minimal (see \cite{bowditch-relhyp}) and hence the $H$-action on the image of the CT 
map is also minimal. Since the limit set of $H$ in $\partial_B G$ is the unique $H$-invariant closed 
set (see e.g. \cite{coornaert}) on which the $H$-action is minimal, the limit set of $H$ in $\partial_B G$ 
is precisely the image of the CT map. Thus the action of $H$ on its limit set in $\partial_B G$ is 
geometrically finite, whence $H$ is relatively quasiconvex (see \cite[Definition 6.2]{hru-rel}). \qed

\smallskip
We note that a statement similar to the second part of Theorem \ref{application 1} can be formulated
in this case too. But it will require more facts about relatively hyperbolic groups to be recalled and
hence we skip it.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Applications to complexes of groups}\label{4}
Complexes of groups are natural generalizations of graphs of groups (see \cite{serre-trees}).
Gerstein and Stallings in \cite{gerstein-stalling} gave the first instances of complexes of groups. 
Subsequently, a more general theory of complexes of groups was studied independently by Corson \cite{corson1} 
and Haefliger \cite{haefliger}. Here, we briefly recall basic facts about some rather special types of complexes 
of groups needed for our purpose. For more details, one is referred to \cite{bridson-haefliger},\cite{haefliger}.

For the rest of this subsection, we shall denote by $\YY$ a finite connected simplicial complex. Let $\BB(\YY)$
denote the directed graph whose vertex set is the set of simplices of $\YY$ and given two simplices $\tau\subset \sigma$
we have a directed edge $e$ from $\sigma$ to $\tau$. In this case we write $e=(\sigma, \tau)$, $o(e)=\sigma$ and $t(e)=\tau$.
Two directed edges $e,e'$ are said to be {\em composable} if $t(e)=o(e')$. In that case the composition
is denoted by $e*e'$.


\begin{defn}[{\bf Complex of groups}] 
A complex of groups $(\mathcal{G},\YY)=(G_{\sigma},\psi_a,g_{a,b})$ over $Y$ consists of the following data:
	\begin{enumerate}
		\item For each $\sigma\in V(\BB(\YY))$, there is a group $G_{\sigma}$- called the local group at $\sigma$.
		
		\item For each edge $e\in E(\BB(\YY))$, there is an injective homomorphism $\psi_e:G_{i(e)}\rightarrow G_{t(e)}$.
These homomorphisms are referred to as the local maps.
		
		\item For each pair of composable edges $e,e'\in E(\BB(\YY))$, a twisting element $g_{e,e'}\in G_{t(e)}$ with the following properties:
		
		(i) $Ad(g_{e,e'})\psi_{e*e'}=\psi_e\psi_{e'}$ where $Ad(g_{e,e'})$ denotes the conjugation by $g_{e,e'}$,
		
		(ii)(Cocycle condition) $\psi_e(g_{e',e''})g_{e,e'*e''} = g_{e,e'}g_{e*e',e''}$ for each triple 
$e,e',e''$ of composable edges of $E(\BB(\YY))$. 
	\end{enumerate} 
\end{defn}
The cocycle condition is empty if dimension of $\YY$ is $2$. If $\YY$ is $1$-dimensional then the complex of groups over $\YY$ 
is the same as the graph of groups over $\YY$. However, given a complex of groups one can define
a complex of space.




\begin{defn} [\bf{Complexes of spaces}]\cite[Definition 1.3]{martin1}
A complex of spaces $C(\YY)$ over $\YY$ consists of the following data:
	\begin{enumerate}
		\item For every simplex $\sigma$ of $\YY$, a CW-complex $C_{\sigma}$.
		\item For every pair of simplices $\sigma\subset \sigma'$, an embedding $\phi_{\sigma,\sigma'}:C_{\sigma'}\rightarrow C_{\sigma}$ called a gluing map such that for every $\sigma\subset\sigma'\subset\sigma''$, we have $\phi_{\sigma,\sigma''}=\phi_{\sigma,\sigma'}\phi_{\sigma',\sigma''}$.
	\end{enumerate}
\end{defn}

The {\em topological realization} $|C(\YY)|$ of the complex of spaces $C(\YY)$ is the following quotient space:
\begin{center}
	$|C(\YY)|=(\bigsqcup\limits_{\sigma\subset \YY}\sigma\times C_{\sigma})/_\sim$
\end{center}
Here all $\sigma$'s are given the subspace topology from the Euclidean spaces and 
$(i_{\sigma,\sigma'}(x),s)\\
\sim(x,\phi_{\sigma,\sigma'(s)})$ for $x\in \sigma\subset\sigma'$, 
$s\in C_{\sigma'}$ and $i_{\sigma,\sigma'}:\sigma\hookrightarrow\sigma'$ is the  inclusion.


Given a complex of groups $(\GG, \YY)$ over $\YY$, for each simplex $\sigma$ of $\YY$ one takes any simplicial complex (generally
a $K(G_{\sigma},1)$-space), say $\YY_{\sigma}$, with a base point such that (1) $\pi_1(\YY_{\sigma})\simeq G_{\sigma}$ and (2)
for every pair of simplices $\tau\subset \sigma$ one has a base point preserving continuous map $\YY_{\sigma}\map \YY_{\tau}$ 
which induces the homomorphism $\psi_{(\sigma, \tau)}$ at the level of fundamental groups. 
This defines a complex of spaces over $\YY$. By abuse of terminology we also call the realization, say
$\YB$, of this to be a complex of spaces as well. Note that we have a natural simplicial map $\YB\map \YY$.


The {\bf fundamental group} $\pi_1(\GG,\YY)$ of $(\GG, \YY)$ is defined to be $\pi_1(\YB)$. 
It is a standard consequence of van Kampen theorem that this is independent of the complex of spaces $C(\YY)$ thus chosen.
For a proof of this one is refered to \cite[Remarks, p. 88]{corson}. When the homomorphisms $\pi_1(\YY_{\sigma})\map \pi_1(\YB)$
induced by the inclusion map $\YY_{\sigma}\map \YB$ are injective for all simplices $\sigma$ of $\YY$ then we say 
that the complex of groups $(\GG, \YY)$ is {\bf developable}. (One can also define developable complexes of group 
as in \cite{haefliger-cplx},\cite{bridson-haefliger}. However, these definitions are equivalent by the results 
of \cite[Section 2]{corson}.)%\RED{ref for comparison with other defns}

{\bf Note:} {\em For the rest of the paper we shall always assume that all our complexes of groups are
developable. We shall denote $\pi_1(\GG, \YY)$ by $G$ for the rest of this section.}

\medskip
{\bf Development or universal cover of a developable complex of groups}\\
Suppose $\tilde{\YB}\map \YB$ is a universal cover of $\YB$. Then as in \cite{corson} one considers the composition
$\tilde{\YB}\map \YB\map \YY$, say $f$, and collapses the connected components of $f^{-1}(y)$ for all $y\in \YY$.
The resulting simplicial complex, say $B$, is called the {\em development} or the {\em universal cover} of 
$(\GG, \YY)$.  Note that $\tilde{\YB}$ has an induced simplicial complex structure from $\YB$ so that the map 
$\tilde{\YB}\map \YB$ is simplicial. Then it follows that $B$ is also a simplicial complex and the natural map 
$B\map \YB$ is simplicial. Moreover, one may show that the development is independent of the complex of spaces chosen for the complex
of groups; see \cite[Section 2]{corson} for a proof. It is in fact the following (see \cite{martin-univ}) simplicial complex:

	\begin{center}
		$B:=(G\times (\bigsqcup\limits_{\sigma\subset Y}\sigma))/\sim$
	\end{center}
	where $(gg',x)\sim (g,x)$ for $g\in G,g'\in G_{\sigma}$, $x\in \sigma$ and 
$(g,i_{\sigma',\sigma}(x))\sim (ge,x)$ for $g\in G,x\in \sigma$ where $i_{\sigma',\sigma}:\sigma'\hookrightarrow \sigma$ is the inclusion map and $e=(\sigma,\sigma')$.

From either of the descriptions of the development it follows that $G$ has a natural simplicial action on $B$ with quotient $\YB$.

%\RED{Shall we remove theorem?}
%\begin{theorem}
%	\textup{(\cite[Theorem 3.13, III.C]{bridson-haefliger})}\label{development} The universal cover of a developable complex of groups $(G,Y)$ is connected and simply connected.
%\end{theorem}
{\bf Notation.} In the remaining part of the paper, $X$ will denote $\tilde{\YB}$ and  $p:X\map B$ will denote the
natural quotient map. 

\begin{rem}\label{remk cplx}
(1) However, we do not work with the CW topology on $B$. We rather view $B$ as the quotient metric space (see \cite[Chapters I.5, I.7]{bridson-haefliger}
obtained by gluing standard Euclidean simplices. Then clearly the $G$-action on $B$ is through isometries.

(2) When $\mathbb Y$ is a finite CW or simplicial complex then we can put a length metric on $\mathbb Y$ 
\cite[Chaper I.7]{bridson-haefliger} which then naturally gives rise to a length metric on $X$ 
\cite[Definition 3.24, Chapter I.3]{bridson-haefliger} and $X$ becomes a geodesic metric space
and the $G$-action on $B$ is (properly discontinuous, cocompact and) through isometries. Also, in this case the map
$p:X\map B$ is $1$-Lipschitz and $G$-equivariant.

(3) In case all the face groups are hyperbolic, one can choose a complex of spaces $C(\YY)$ where the spaces for each
face is a finite CW or simplicial complex since hyperbolic groups are finitely presented. Thus $|C(\YY)|$ a finite
CW (or simplicial) complex.
\end{rem}

The following proposition follows from \cite[Theorem 5.1]{charney-crisp}. For an alternative treatment one may look
up \cite[Section 3]{mbdl2}. 
\begin{prop}\label{development is cone off}
Let $\YY$ be a finite simplicial complex and let $(\GG,\YY)$ be a developable complex of groups. Let $p: X\map B$ be
as in (2) of the Remark \ref{remk cplx}.
Suppose $x\in X$. Consider the orbit map $\mathcal O: G\map X$ given by $g\mapsto g.x$.
%which is a quasiisometry by Milnor-Svarc theorem. 
There is a constant $D\geq 0$ such that the following holds: \\Let $g\in G$, $\sigma\subset \YY$ be a face and 
$y\in \sigma$ is the barycenter of $\sigma$.

Then (1) $Hd(\mathcal O(gG_{\sigma}), p^{-1}([g,y]))\leq D$ where $[g,y]$ denotes the equivalence
class of $(g,y)$ in $B$ as defined above.

(2) The spaces obtained from $X$ by coning off the following two collections of subsets are naturally quasiisometric:

\noindent
(i) Inverse images of all points in $B$ under $p$.\\
(ii) Inverse images under $p$ of only the barycenters of the various simplices of $B$.

(3) The map $p\circ \mathcal O$ induces a $G$-equivariant quasiisometry $\hat{G}\map B$ where $\hat{G}$ is the coned off
Cayley graph of $G$ obtained by coning the various cosets of the face groups of $(\GG, \YY)$.
\end{prop}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




Following is the set up for the main theorem of this section.

\begin{itemize}
\item (H1) Suppose $(\mathcal{G},\YY)$ is a developable complex of groups %with qi embedding condition with $\pi_1(\GG, Y)=G$
with the development $B$.
\item (H2) Suppose $G$ is hyperbolic and all the face groups are quasiconvex in $G$. 
%Then it follows that $B$ \RED{explain} is a hyperbolic metric space.
\item (H3) Suppose $\YY_1$ is a connected subcomplex of $\YY$ and $(\mathcal{G},\YY_1)$ is the subcomplex of groups 
obtained by restricting $(\mathcal{G},\YY)$ to $\YY_1$. Then by \cite[Corollary 2.15, Chapter III.C]{bridson-haefliger}
$(\mathcal{G},\YY_1)$ is a developable complex of
groups. Let $G_1=\pi_1(\GG, \YY_1)$ and let $B_1$ be the development. 
\item (H4) Suppose the natural homomorphism $G_1\map G$ is injective. Then we have a natural map $B_1\map B$.
\item (H5) Suppose $G_1$ is also hyperbolic. 
\end{itemize}
Then we have the following.

\begin{theorem}\label{acyl ct thm}
(1) The spaces $B, B_1$ are hyperbolic.

(2) If the natural map $B_1\rightarrow B$ satisfies Mitra's criterion
then there exists a Cannon-Thurston map for the inclusion $G_1\rightarrow G$. 
Moreover, $G_1$ is quasiconvex in $G$ if and only if the Cannon-Thurston map for 
$B_1\rightarrow B$ is injective.
\end{theorem}
\proof Let $C(\YY)$ be a complex of spaces for the complex of groups $(\mathcal{G},\YY)$
where the space for each simplex is a finite simplicial complex. Let $C(\YY_1)$
be the restriction of $C(\YY)$ to $\YY_1$. Let $\mathbb Y$ be the topological realization
of $C(\YY)$ and let $\mathbb Y_1$ be the topological realization of $C(\YY_1)$.
Then we have the following commutative diagram (figure \ref{pic 1}) where the horizontal
maps are inclusions.

\begin{figure}[h]
	\[ \begin{tikzcd}[column sep=4.2em,row sep=3.2em]
		\mathbb{Y}_1 \arrow{r} \arrow[swap]{d} & \mathbb{Y} \arrow{d} \\%
		\YY_1\arrow{r} & \YY
	\end{tikzcd}
	\]
	\caption{}
	\label{pic 1}
\end{figure}

 %\RED{draw diagram}

Let $f:X\map \mathbb Y$ and $f_1:X_1\map \mathbb Y_1$ be universal covers.
Then we have a commutative diagram as below where the top horizontal map
can be assumed to be an inclusion map since $\pi_1(\YB_1)\map \pi_1(\YB)$ is injective.

\begin{figure}[h]
	\[ \begin{tikzcd}[column sep=4.2em,row sep=3.2em]
		X_1 \arrow{r} \arrow[swap]{d}{f_1} & X \arrow{d}{f} \\%
		\mathbb{Y}_1\arrow{r} & \mathbb{Y}
	\end{tikzcd}
	\]
	\caption{Horizontal maps are inclusion}
	\label{pic 2}
\end{figure}
%\RED{draw diagram}

Since the top horizontal map is $G_1$-equivariant by choosing $x\in X_1$ and using 
Proposition \ref{development is cone off} we have a commutative diagram
as below. 

\begin{figure}[h]
	\[ \begin{tikzcd}[column sep=4.2em,row sep=3.2em]
		\hat{G_1} \arrow{r} \arrow[swap]{d} & \hat{G} \arrow{d} \\%
		B_1\arrow{r} & B
	\end{tikzcd}
	\]
	\caption{Vertical maps are quasiisometries}
	\label{pic 3}
\end{figure}

%\RED{draw}

Here the vertical maps are quasiisometries. Hence, (1) follows  %$B$ and $B_1$ are hyperbolic
from Proposition \ref{mj-dahmani} and also $B_1\map B$ admits the CT map or satisfies Mitra's
criterion if and only if the same is true for the map $\hat{G}_1\map \hat{G}$. Moreover, any of these two maps is injective if and only if
so is the other one. Hence, the first part of (2) in the theorem follows from the first part of Theorem \ref{application 1}(1).
It also follows that in this case the CT map $\partial G_1\map \partial G$ is injective if and only if
so is the CT map $\partial B_1\map \partial B$. Thus the second part of (2) follows from the second part of
Theorem \ref{application 1}(1). \qed

\smallskip
Below we mention two instances of complexes of groups where the fundamental groups are
hyperbolic and all the face groups are quasiconvex.

\subsubsection{Complexes of groups with finite edge groups}
In this section we consider developable complexes of groups whose edge groups are finite and whose developments are hyperbolic
which may or may not be CAT(0).
The following proposition then is immediate from the work of \cite{bowditch-relhyp}, and \cite{pedroja-fine-graph}. We include the statement
in this paper because we could not find it in the literature.

\begin{theorem}\label{gen fin edge}
Suppose $(\GG,\YY)$ is a developable complex of groups such that the edge groups are finite and the universal cover of $(\GG,\YY)$ is a hyperbolic
metric space. Then the fundamental group of $(\GG,\YY)$, say $G$, is hyperbolic relative to the vertex groups $\{G_v: v\in V(\YY)\}$.
\end{theorem}
{\em A word about the proof:} Bowditch (\cite{bowditch-relhyp}) showed that a finitely generated group is hyperbolic relative 
to a finite set of finitely generated infinite subgroups $\{H_i\}$ if and only if there is a {\em fine} hyperbolic graph $X$ on which 
$G$ has a cofinite action and such that the edge stabilizers
are finite and the infinite vertex stabilizers are precisely the conjugates of $\{H_i\}$ in $G$. Using this criterion one 
only needs to check that the $1$-skeleton of the development of $(\GG, \YY)$ is a fine graph. 
This follows from \cite[Corollary 2.11, Theorem 1.3]{pedroja-fine-graph}. %\RED{exact theorem no?}


Now, in the above theorem if one assumes in addition that the vertex groups are hyperbolic then one has the following:

\begin{theorem}\label{combhyp finite edge}
Suppose $(\GG,\YY)$ is a developable complex of groups such that the vertex groups are hyperbolic and the edge groups are finite. 
Suppose the universal cover of $(\GG,\YY)$ is  hyperbolic. Then the fundamental group of $(\GG,\YY)$ is a hyperbolic group
and vertex groups are quasiconvex in $G$.
\end{theorem}
In fact, one may use Theorem \ref{gen fin edge} along with \cite[Corollary 2.41]{osin-book} or \cite[Theorem 2.4]{hamnestadtrelative}
for the proof of Theorem \ref{combhyp finite edge}.

%\begin{rem}
%In Theorem \ref{combhyp finite edge}, we can not drop 	the hypothesis that the universal cover of complex of hyperbolic groups is a hyperbolic space, see \cite[Example 12.17(3), II.12]{bridson-haefliger}. In that example, we have a developable triangle of finite groups $(\GG,\YY)$ whose universal cover is the Euclidean space $\mathbb{E}^2$. Since $\pi_1(\GG,\YY)$ is quasiisometric to $\mathbb{E}^2$, $\pi_1(\GG,\YY)$ is not a hyperbolic group.
%\end{rem}

Here is the set up for the main result of this subsection.
\begin{itemize}
\item Suppose $(\GG,\YY)$ is a complex of groups as in Theorem \ref{gen fin edge} with $\pi_1(\GG,\YY)=G$
and with universal cover $B$. 
\item Suppose $\YY_1\subset \YY$ is a connected subcomplex and $(\GG,\YY_1)$ is the restriction of $(\GG,\YY)$ to $\YY_1$ such that at the level 
of fundamental groups we have an injection. 
Let $H=\pi_1(\GG,\YY_1)$ and let $B_1$ be the universal cover of $(\GG,\YY_1)$. 
\item Assume that $B_1$ is hyperbolic.
We note that this implies $H$ is hyperbolic relative to the vertex groups in $(\GG,\YY_1)$ by
Theorem \ref{gen fin edge}.

\end{itemize}
Then, by Theorem \ref{application 2} we have the following:

\begin{theorem}
There is a Cannon-Thurston map $\partial_{rel} H\map \partial_{rel} G$ at the level of the Bowditch boundaries of $H$ and
$G$ if Mitra's criterion holds for the inclusion $B_1\map B$.

Moreover, $H$ is a relatively quasiconvex subgroup of $G$ if and only if the CT map for $B_1\map B$ is injective.
\end{theorem}
Similarly, by Theorem \ref{application 1} we immediately have the following:
\begin{theorem}
Suppose $(\GG,\YY)$ satisfies the hypotheses of Theorem \ref{combhyp finite edge}.  Then
	there is a Cannon-Thurston map $\partial H\map \partial G$ at the level of the Gromov boundaries of $H$ and
	$G$ if Mitra's criterion holds for the inclusion $B_1\map B$.
	
	Moreover, $H$ is quasiconvex in $G$ if and only if the CT map for $B_1\map B$ is injective.
\end{theorem}
\begin{comment}
\proof \RED{The proof needs more preparation: define rel qc, rel cayley graph, equiv of defns of rel qc}
The first part follows immediately from Theorem \ref{application 2} and Theorem \ref{combhyp finite edge}.
Suppose $H$ is a relatively quasiconvex subgroup of $G$. Then by \cite[Theorem 9.1]{hru-rel}, 
$H$ is a relatively hyperbolic group 
with respect to infinite vertex groups of $(\GG,Y_1)$. Again, by \cite[Theorem 10.1]{hru-rel}, the natural inclusion $H\rightarrow G$ 
induces a qi embedding between relative Cayley graphs of $H$ and $G$, respectively. But we know that relative Cayley graph is quasiisometric to coned-off Cayley graph (see \cite{osin-book}). Also, coned-off Cayley graphs of $G,H$ with respect to peripheral structure are quasiisometric to $B,B_1$, respectively. Hence, there exists a qi embedding from $B_1$ to $B$.
	
	Conversely, suppose that the inclusion $B_1^{(1)}\rightarrow B^{(1)}$ is a qi embedding. Above, we saw that the $1$-skeleton of $B$ is a fine hyperbolic graph. Now, $B^{(1)}$ is a qi embedded subgraph of $1$-skeleton of $B$ and also it is $H-$invariant. Hence by \cite[Definition 1.3]{pedraoja-wise}, we see that $H$ is a relatively quasiconvex subgroup of $G$. 
\qed
\end{comment}

\subsubsection{Acylindrical complexes of groups}

In \cite{martin1} (along with \cite[Corollary, p. 805]{martin-univ}) A. Martin proved the following theorem for complexes of 
hyperbolic groups. %\RED{Give theorem no.s along with citation in the theorem below.}

\smallskip
{\bf Theorem} \textup{(\cite[p. 34]{martin1}\label{martin})} {\em Let $(\mathcal{G},\YY)$ be a developable complex of groups such that
the following holds:
\begin{itemize}
\item (M1) $\YY$ is a finite connected simplicial complex,
\item (M2) all the face groups are hyperbolic and local maps are quasiisometric embeddings,
\item (M3) the universal cover of $(\mathcal{G},\YY)$ is a CAT(0) hyperbolic space, and
\item (M4) the action of $\pi_1(\mathcal{G},\YY)$- the fundamental group of $(\mathcal{G},\YY)$, on the
development is acylindrical.
\end{itemize} 
Then $\pi_1(\mathcal{G},\YY)$ is a hyperbolic group and the local groups are quasiconvex in $\pi_1(\mathcal{G},\YY)$.}

\smallskip
In what follows, the above theorem is referred to as Martin's theorem. Using this theorem we deduce the following corollary to Theorem \ref{acyl ct thm}.

\begin{cor}\label{martin application}
Let $(\mathcal{G},\YY)$ be a complex of groups satisfying the conditions (M1)-(M4) of the above theorem. 
Let $\YY_1$ be a connected subcomplex of $\YY$ and 
let $(\mathcal{G},\YY_1)$ be the subcomplex of groups obtained by restricting $(\mathcal{G},\YY)$ to $\YY_1$. Suppose 
the following conditions hold:

\begin{enumerate}
\item $(\mathcal{G},\YY_1)$ also satisfies (M1)-(M4),
\item the natural homomorphism $H=\pi_1(\mathcal{G},\YY_1) \map G=\pi_1(\mathcal{G},\YY)$ is injective,
\item  the natural map  $B_1\rightarrow B$ satisfies Mitra's criterion where $B_1,B$ are the universal covers
of $(\mathcal{G},\YY_1)$ and $(\mathcal{G},\YY)$ respectively. 
\end{enumerate}

Then there exists a Cannon-Thurston map for the inclusion $H\rightarrow G$. 
Moreover, $H$ is quasiconvex in $G$ if and only if the Cannon-Thurston map for $B_1\rightarrow B$ is injective.
\end{cor}



\section{Other applications and examples}\label{5}

In this section we prove a few other related results about complexes of groups. 
%Here is the set-up for the first theorem.


\subsection{Polygons of groups} %Let $Y$ be a regular Euclidean polygon with at least $4$ edges. Let $(\GG,Y)$ be a simple (i.e. all twisting elements are trivial) polygon of groups over $Y$. Also, assume that in vertex groups, the intersection of the two subgroups coming from the incident edges is equal to the subgroup coming from the barycenter of $Y$. Let $G=\pi_1(\GG,Y)$.
%Unless stated otherwise, this will be our standing assumption for the rest of this subsection. 

Following is the main result of this subsection that we obtain as an application of Theorem \ref{acyl ct thm}.

\begin{theorem}\label{edge qc}
Suppose $\mathcal{Y}$ is a regular Euclidean polygon with at least $4$ edges and let $(\GG,\YY)$ be a simple complex of hyperbolic groups
such that the following are satisfied:
\begin{enumerate}
\item In any vertex group, intersection of two different edge groups is equal to the subgroup coming from the barycenter of $\YY$. 
%%$G=\pi_1(\GG,Y)$. all the local groups of $(\GG,Y)$ are hyperbolic and all the local maps are qi embeddings. 
\item The universal cover $B$ of $(\GG,\YY)$ is a hyperbolic metric space.
\item The action of $G=\pi_1(\GG,\YY)$ on $B$ is acylindrical. 
\end{enumerate}

Suppose $\YY_1$ is an edge of $\YY$ and $(\GG,\YY_1)$ is the restriction of $(\GG,\YY)$ to $\YY_1$. Let $H=\pi_1(\GG,\YY_1)$.
Then $G$ is a hyperbolic group and $H$ is a quasiconvex subgroup of $G$.
\end{theorem} 

\proof We begin with the following simple observation.
By \cite[12.29, p. 390, II.12]{bridson-haefliger}, $(\GG,\YY)$ is non-positively curved and 
hence it is developable. Also
$B$ is a piecewise Euclidean polygon complex, and by \cite[Theorem 7.50, I.7]{bridson-haefliger}
$B$ is a complete geodesic metric space since all simplices are isometric to each other.
It follows that $B$ is a CAT(0) space (see \cite[paragraph after Theorem 4.17, p. 562, III.C]{bridson-haefliger}). 
Thus all the hypotheses of Martin's theorem are satisfied for $(\GG,\YY)$ and hence $G$ is a hyperbolic group.

Next part of the proof makes use of the following three lemmas. We shall need the following definition. 
Let $d$ denote the metric on $B$ and let $d_P$ denote the metric on any polygon $P$ in $B$. We also assume that each edge in $B$ is of length $1$.

%Next, we adapt the following definition from  to our context.
\begin{defn}{\em (\cite[Chapter I.7, Definition 7.8]{bridson-haefliger})}
	Suppose $x\in B$. Define $$\epsilon(x)=\inf\{\epsilon(x,P): \text{$P$ is a polygon in $B$ containing $x$} \}$$
	where $\epsilon(x,P):=\{d_P(x,e):e \text{ is an edge of $P$ not containing $x$}\}$.
\end{defn}
The lemma below can be proved in the same way as \cite[Lemma 7.9]{bridson-haefliger}. 
For the sake of completeness, we include a sketch of proof. %By an $m$-string in $B$ we mean the same as in \cite[I.7, Definition 7.4]{bridson-haefliger}.

\begin{lemma}\label{pologon lemma 1}
	Fix $x\in B$. If $y\in B$ is such that $d(x,y)< \epsilon(x)$ then any polygon $P$
	which contains $y$ also contains $x$ and $d(x,y)= d_P(x,y)$.
\end{lemma}
{\em Sketch of proof:} To prove the lemma, it is sufficient to show that if 
$\Sigma=(x=x_0,x_1,...,x_n=y)$ is an $m$-string (see \cite[I.7, Definition 7.4]{bridson-haefliger}) 
of length $l(\Sigma)<\epsilon(x)$, with $m\geq 2$, then $\Sigma'=(x_0,x_2,...,x_n)$ is an $(m-1)$-string 
with length $l(\Sigma')\leq l(\Sigma)$. Now, by definition of $m$-string, there is a polygon $P_1$ such 
that $x_1,x_2\in P_1$. Since $l(\Sigma)< \epsilon(x)$, $x_0\in P_1$. By triangle inequality, 
$d_{P_1}(x_0,x_2)\leq d_{P_1}(x_0,x_1)+d_{P_1}(x_1,x_2)$. Thus, $(x_0,x_2,...,x_n)$ is an 
$(m-1)$-string of length less that or equal to $l(\Sigma)$.  \qed

\smallskip
The following lemma must be well known or obvious but we could not find a written proof anywhere in the literature.
Hence we include a proof here.
\begin{lemma}\label{iso. embedd. poly.}
	The inclusion of any polygon $P$ in $B$ is an isometric embedding where $P$ is given its Euclidean metric.
\end{lemma}
\proof
Suppose $x,y\in P$ are two interior points and $[x,y]_P$ is the straightline joining $x,y$ in $P$.
For all $z\in [x,y]_P$ the ball of radius $\epsilon(z)$ in $P$ is isometrically embedded in $B$ by Lemma \ref{pologon lemma 1}.
Hence, a small neighborhood of $z$ in $[x,y]_P$ is isometrically embedded in $B$. This shows that $[x,y]_P$ is a local
geodesic in $B$. Since $B$ is a CAT(0) space, it follows that $[x,y]_P$ is a geodesic in $B$. Thus the interior of $P$
is isometrically embedded in $B$. 
%On the it is clear that the inclusion $P\map B$ is a Lipschitz map whence the closure in $B$ of the interior of $P$. 
The lemma follows easily from this and the following standard fact (see \cite[Proposition 1.4(1), II.1]{bridson-haefliger}):\\ 
 {\em Suppose $\{z_n\},\{z'_n\}$
are two sequences in a CAT(0) space $Z$ and $z,z'\in Z$ such that $z_n\map z, z'_n\map z'$. Let 
$\alpha_n:[0,1]\map Z$ be a constant speed geodesic joining  $z_n,z'_n$ in $Z$ for all $n\in \NN$. Then $\alpha_n$ converges 
uniformly to a constant speed geodesic $\alpha:[0,1]\map Z$ joining $z,z'$.} \qed
\begin{comment}
Let $P$ be a polygon in $B$ and let $x,y\in P$. We want to show that the geodesic $[x,y]_P$ joining $x,y$ in $P$
is also a geodesic in $B$. The proof is divided into several cases:

{\bf Case 1.} \underline{Suppose $x,y$ are both interior points of $P$.}
Let $z\in [x,y]_P$. Then the ball of radius $\epsilon(z)$ in $P$ is isometrically embedded in $B$ Lemma \ref{pologon lemma 1}.
Hence, a small neighborhood of $z$ in $[x,y]_P$ is isometrically embedded in $B$. This shows that $[x,y]_P$ is a local
geodesic in $B$. Since $B$ is a CAT(0) space, it follows that $[x,y]_P$ is a geodesic.

 be an interior point of $P$. Then, by Lemma \ref{pologon lemma 1}, an open $P$-ball of radius $\epsilon(x)$ around $x$ embeds isometrically in $B$. Firstly, we show that the interior of $P$ embeds isometrically in $B$. Let $x,y$ be any two points in the interior of $P$ and let $\alpha$ be the $P$-geodesic connecting $x$ and $y$. To show that $\alpha$ is a geodesic in $B$, it is sufficient to show that it is a local geodesic in $B$ since in a CAT(0) space a local geodesic is a geodesic. Let $z\in Im(\alpha)$ be any point. Then $B_P(z,\epsilon(z))\cap \alpha$ embeds isometrically in $B$. Thus $\alpha$ is a local geodesic in $B$. Now, let $x$ be an interior point of $P$ and let $y$ be a point on a side of $P$. Let $\beta$ be the $P$-geodesic joining $x$ and $y$. Then there is a sequence $\{x_n\}$ in the interior of $P$ such that $x_n\in\beta$ and $x_n\map y$ in $P$. Since the inclusion $P\map B$ is $1$-Lipschitz, $x_n\map y$ in $B$ too. Now, $\lim_{n\map \infty}d_B(x,x_n)=d_B(x,y)$ and $\lim_{n\map \infty}d_P(x,x_n)=d_P(x,y)$. But $d_P(x,x_n)=d_B(x,x_n)$. Thus, $d_P(x,y)=d_B(x,y)$. Similarly, it can be shown that if $x$ and $y$ lie on distinct sides of $P$ then $d_P(x,y)=d_B(x,y)$. Finally, suppose $x\neq y$ are two vertices on a side, say $e$, of $P$. Let $e'\neq e$ be a side of $P$ having $y$ as a vertex. Suppose $\{x_n\in e'\}$ is a sequence such that $x_n\map y$ in $P$. This implies that $x_n\map y$ in $B$ too. As in the previous case, $d_P(x,x_n)=d_B(x,x_n)$. Also, $\lim_{n\map \infty}d_P(x,x_n)=d_P(x,y)$ and $\lim_{n\map \infty}d_B(x,x_n)=d_B(x,y)$. Hence $d_P(x,y)=d_B(x,y)$. This completes the proof.
\end{comment}

%\RED{It seems that you are using the fact that each edge is of length 1 in the following proof. This needs explanation.}
\begin{lemma}\label{polygon lemma 2}
	Let $P_1$ and $P_2$ be two distinct polygons in $B$. Suppose $e_1\subset P_1$ and $e_2\subset P_2$ are edges
such that $e_1\cap P_2=e_2\cap P_1=e_1\cap e_2$ is a vertex. Then the concatenation of $e_1$ and $e_2$ is a geodesic in $B$.
\end{lemma}
\begin{proof}
	 Let $\alpha$ be the concatenation of $e_1$ and $e_2$. By Lemma \ref{iso. embedd. poly.}, $e_1,e_2$ are geodesics in $B$. 
Let $v:= e_1\cap e_2$. To prove the lemma, it is sufficient to show that a small neighborhood of $v$ in $\alpha$ embeds 
isometrically in $B$. Let $I$ be the open ball of radius $1/4$ around $v$ in $\alpha$. Suppose $x,y$ are the endpoints 
of $I$ lying in $e_1,e_2$ respectively. Note that $\Sigma_0=(x,v,y)$ is a $2$-string in $B$ and $l(\Sigma_0)=1/2$. 
If there is no string in $B$, except $\Sigma_0$, connecting $x$ and $y$ then we are done. Therefore, we show that if 
$\Sigma=(x_0=x,x_1,...,x_n=y)$ is any other $n$-string in $B$ then $l(\Sigma)>l(\Sigma_0)$. By definition of an $n$-string, 
there exists a sequence of polygons, say $(P_0',P_1',...,P_{n-1}')$, such that $x_i,x_{i+1}\in P_i'$ for $i=0,1,...,(n-1)$.
 Without loss of generality, we can assume that $x_i,x_{i+1}$ lie on different sides of $P_i'$ for $0\leq i\leq (n-1)$. Note 
that if $x_1$ belongs to a side of $P_0'$ not containing $v$ then $d_{P_0'}(x,x_1)>1/2$ as the angle at each vertex 
of $P_0'$ is at least $\pi/2$ and hence $l(\Sigma)>1/2$. Thus we assume that $x_1$ belongs to a side of 
$P_0'$, say $e_3$, containing $v$. Since the angle between $e_1$ and $e_3$ is at least $\pi/2$, 
$d_{P_0'}(x,x_1)> 1/4$. By the same reasoning, $x_2$ belongs to a side of $P_1'$ containing $v$. By continuing in 
this way either $x_{n-1}$ belongs to a side of $P_{n-1}'$ containing $v$ or $x_{n-1}$ lies on a side of $P_{n-1}'$ not 
containing $v$. In either case $d_{P_{n-1}'}(x_{n-1},x_n)>1/4$. Hence, 
$l(\Sigma)\geq d_{P_0'}(x,x_1)+d_{P_{n-1}'}(x_{n-1},x_n)>1/2$. This completes the proof.
\end{proof}


{\em Proof of Theorem \ref{edge qc} continued:}
	Let $v,w$ be the vertices and $e$ the barycenter of $Y_1$. 
Then $H=G_v\ast_{G_e}G_w$. Let $B_1$ denote the Bass-Serre tree for the amalgam decomposition of $H$. 
	%Then $B_1$ is a CAT(0) space. %On $B$, we have a piecewise Euclidean metric and it is a complete geodesic metric space 
	%(see \cite[I.7]{bridson-haefliger}). With this metric, from the above discussion, $B$ is also a CAT(0) space. 
We note that there is a natural homomorphism $H\map G$ and a natural simplicial map $B_1\map B$.

{\bf Claim:} The natural map $B_1\map B$ is an isometric embedding.\\
{\em Proof of Claim.} Since $B$ is a CAT(0) space, it is enough to show that the restriction of the
map $B_1\map B$ to any geodesic of $B_1$ is a local isometry. Let  $\alpha$ be any geodesic
	of $B_1$. Then the edges on $\alpha$ are mapped to geodesics 
in $B$ by Lemma \ref{iso. embedd. poly.}. Thus, the map $\alpha\map B$ is locally isometric at all points of $\alpha$
other than possibly the vertices. Now, suppose $b_1,b,b_2$ are consecutive vertices on $\alpha$.
	We know that vertices and edges of $B_1$ and $B$ correspond to cosets of vertex and edge groups in $H$ and $G$ respectively,
	and the $2$-dimensional faces of $B$ correspond to cosets of $G_{\tau}$ in $G$, where $\tau$ is the $2$-dimensional face of $Y$	(see \cite[Theorem 2.13, Chapter III.C]{bridson-haefliger}). %\RED{very unclear after this}
 Since the map $B_1\map B$ is equivariant under the homomorphism $H\map G$
and there are only two orbits of vertices  and one orbit of edges under the $H$-action, we may assume
without loss of generality that  $b$ corresponds to the local group $G_v$ (i.e.
the stabilizer of the vertex $b$ of $\alpha$ is $G_v$), $b_1$ correspond to the $G_w$ and 
$b_2$ correspond to $g_vG_w$, where $g_v\in G_v\setminus G_e$. We note the following. (1) $g_v\not \in G_{\tau}$, (2) $b,b_1$ are in
the $2$-dimensional face corresponding to $G_{\tau}$, but (3) $b,b_2$ are in the $2$-dimensional face
corresponding to $g_vG_{\tau}$. Consequently the edges $[b,b_1]$ and $[b,b_2]$ lie in two distinct polygons
in $B$ and satisfy the hypotheses of Lemma \ref{polygon lemma 2}. 
Hence, the concatenation of these edges is a geodesic in $B$. This proves that the inclusion $B_1\map B$ is
an isometric embedding.

It then follows that (1) the homomorphism $H\map G$ is injective; (2) the $H$-action on $B_1$ is acylindrical,
since $G$-action on $B$ is acylindrical. Hence, $H$ is a hyperbolic group by \cite[Theorem 3.7]{ilyakapovichcomb}.
Also since $B_1\map B$ is an isometric embedding Mitra's criterion clearly holds, and the CT map $\partial B_1\map \partial B$
is injective by Lemma \ref{bdry basic prop}(3). Thus all the hypotheses of Theorem \ref{acyl ct thm} are verified. Hence, 
$H$ is quasiconvex in $G$.
\qed

\begin{rem}
(1) Theorem \ref{edge qc} is false for a triangle of groups in general. In this case, the natural homomorphism 
$\pi_1(\GG,\YY_1)\rightarrow \pi_1(\GG,\YY)$ need not even be injective. However, if $\YY$ is a polygon with at least $4$ edges 
and if $(\GG,\YY)$ satisfies the condition (1) of Theorem \ref{edge qc} then it follows that $(\GG,\YY)$ is developable
\RED{cite} and that the natural homomorphism $\pi_1(\GG,\YY_1)\rightarrow \pi_1(\GG,\YY)$ is injective. For the latter see the proof of Corollary 
\ref{graph qc}(1) below.  

Even there are examples of developable triangles of groups such that development is a CAT(0) hyperbolic space, the fundamental group $G$ of the triangle of groups is hyperbolic, but amalgamated free product corresponding to an edge is not quasiconvex in $G$, see Example \ref{not qc edge}.
	
(2) Let $\YY$ be an Euclidean polygon with at least $4$ edges. Suppose $(\GG,\YY)$ is a developable simple polygon of groups. Then $(\GG,\YY)$ satisfy the conditions (M2)-(M4) of Martin's theorem if and only if $(\GG,\YY)$ satisfies the hypotheses of Theorem \ref{edge qc}.
\end{rem}



Next we obtain a generalization of Theorem \ref{edge qc} as follows.
Suppose $(\GG,\YY)$ is a polygon of groups as in Theorem \ref{edge qc},
Suppose $\YY_2$ is a connected subgraph of the boundary of $\YY$ consisting of $n-3$ edges.
Suppose $v,w\in \YY$ are the two vertices in the complement of $\YY_2$. 
Let $J$ be the line segment inside $\YY$ joining midpoints of the edges incident on $v$ and $w$ respectively on
the opposite side of the edge $[v,w]$. Let $\YY_1$ be the edge $[v,w]$.
Let $G_1=\pi_1(\GG,\YY_1)$ and $G_2=\pi_1(\GG, \YY_2)$. Let $e_1,e_2$ be the edges incident on $v,w$ respectively
whose midpoints are joined by $J$. Let $\tau$ denote the barycenter of $\YY$ as before. 
Suppose $K=G_{e_1}\ast_{G_\tau}G_{e_2}$ be the natural amalgamated free product for the monomorphisms
$G_{\tau}\map G_{e_i}$, $i=1,2$. 
Note that we can realise $K$ as a subgraph of groups of $(\GG,\YY_1),(\GG,\YY_2)$ respectively. \RED{explain}
Hence, there are the natural homomorphisms $K\map G_i$, $i=1,2$. Now we have the following corollary to
Theorem \ref{edge qc}.

\begin{cor}\label{graph qc}
(1) The homomorphisms $K\map G_i$, $i=1,2$ are injective whence we have an amalgam decomposition
$G=G_1*_K G_2$.

(2) $G_1,G_2, K$ are all quasiconvex subgroups of $G$.

(3) If $\YY'$ is any connected subgraph of $\YY_2$ then $G'=\pi_1(\GG,\YY')$ is quasiconvex in $G$.
\end{cor}

We need a little preparation for the proof of the corollary.


In \cite{GMRS}, Gitik et al. generalized the concept of malnormality and introduced the following notion of {\em height} of a subgroup of a group. 
%Let $H$ be a subgroup of a group $G$. The elements $\{g_i\}$ in $G$ are said to {\em essentially distinct} if for, $i\neq j$, the cosets $g_iH$ and $g_jH$ are distinct. Conjugates of $H$ by essentially distinct elements are called {\em essentially distinct conjugates}.
\begin{defn}
	[Height]  The height of an infinite subgroup $H$ in $G$ is the maximal $n\in\mathbb{N}$ such that if there
	exists distinct cosets $g_1H,g_2H,...,g_nH$ such that $g_1Hg_1^{-1}\cap g_2Hg_2^{-1}\cap...\cap g_nHg_n^{-1}$ is infinite.
	The height of a finite subgroup define to be $0$.
\end{defn}
In \cite{GMRS}, the authors proved the following:
\begin{theorem}\textup{(\cite[p. 322]{GMRS})}\label{finite height of qc}
	Quasiconvex subgroups of hyperbolic groups have finite height.
\end{theorem}

The following lemma is a simple consequence of Bass-Serre theory and hence we skip its proof.
\begin{lemma}\label{finite height implies acyl}
	Suppose $(\GG,\YY)$ is a finite graph of groups with fundamental group $G$. If all the edge groups have finite height in $G$ then the action of $G$ on the Bass-Serre tree of $(\GG,\YY)$ is acylindrical.
\end{lemma}

{\em Proof of Corollary \ref{graph qc}.}
(1) follows from the results in \cite[2.15, p.25]{basscovering} since $K$ can be naturally
identified as the fundamental group of a subgraph of groups of $(\GG,\YY_i)$, $i=1,2$.
%We show that the homomorphism $\pi_1(\GG,Y')\map G$ is a qi embedding and deduce the corollary from this.

	
(2) We know that $G$ is a hyperbolic group and all vertex groups are uniformly quasiconvex in $G$ and also
$G_1$ is quasiconvex in $G$ by Theorem \ref{edge qc}. It follows that all the vertex groups of $G$ 
have finite height by Theorem \ref{finite height of qc}. Hence, all the vertex groups of $G_2$ have finite height in $G_2$
as well. Hence, $G_2$-action on its Bass-Serre tree is acylindrical by Lemma \ref{finite height implies acyl}.
Thus by \cite[Theorem 3.7]{ilyakapovichcomb} (or by the Martin's theorem) $G_2$ is hyperbolic.

Finally, by \cite[Theorem 8.73]{kapovich-sardar}, the group $K$ is quasiconvex in $G_1$.
By Theorem \ref{edge qc} $G_1$ is quasiconvex in $G$. Hence $K$ is quasiconvex
in $G$. Thus it easily follows that $G_2$ is quasiconvex in $G$. 

(3) Once again by \cite[Theorem 8.73]{kapovich-sardar}
$G'$ is quasiconvex in $G_2$. Thus using (2) $G'$ is quasiconvex in $G$. \qed


\begin{comment}
	Since $(\GG,Y)$ is a finite graph of groups, there exists $l\in\mathbb{N}$ such that the height of each edge group is at most $l$. Let $T$ be the Bass-Serre tree of $(\GG,Y)$. Note that the $G$-stabilizer of a geodesic $\alpha$ in $T$ is the intersection of the $G$-stabilizers of edges on $\alpha$. Let if possible the action of $G$ on $T$ is not acylindrical. Then, given $k\in\mathbb{N}$ there is a geodesic in $T$ with length bigger than $k$ and the $G$-stabilizer of the geodesic is infinite. Now, choose $k$ to be sufficiently larger than $l$ such that there is a geodesic segment $\beta$ of length bigger than $k$ and  the $G$-stabilizer of $\beta$ is infinite. Since there are finitely many edge groups, the $G$-stabilizer of $\beta$ is contained in the intersection of more than $l$-conjugates of an edge group. This gives a contradiction as the height of each edge group is at most $l$.
\end{comment}
%\RED{serious problem in the proof: Why is the hom $G_2\map G$ injective?}
Finally we prove the following application of Corollary \ref{graph qc}.
\begin{prop}\label{virtually special}
	Suppose $(\GG,\YY)$ is a polygon of groups satisfying the hypotheses of Theorem \ref{edge qc}
such that the vertex groups are also virtually compact special. Then $G=\pi_1(\GG,\YY)$ is virtually compact special.
\end{prop}
\proof Let $\YY_1,\YY_2$, $G_1,G_2,K$ be as in Corollary \ref{graph qc}. 
Then $G=G_1*_K G_2$ is virtually compact special by \cite[Theorem 13.1]{wisehierarchy} since
$K$ is quasiconvex in $G$ by Corollary \ref{graph qc}
\qed



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Examples}\label{examples}


%\medskip
We end the paper with two concrete examples which demonstrate the necessity of some of the hypotheses in 
some of the theorems of the previous sections. 


 The first example shows that the natural inclusion from the universal cover of the subcomplex of groups 
to the universal cover of the complex of groups is not always a proper embedding. In particular, it shows that 
the converse of Theorem \ref{acyl ct thm} is not true in general. The second examples show that Theorem
\ref{edge qc} is false for triangles of groups. For the both the examples following is the common set up:

\begin{enumerate}
\item $\YY$ is a triangle as in figure \ref{pic 4} and $(\GG,\YY)$ is a triangle of groups. 
\item We shall denote the local group for any face $\sigma$ by $G_{\sigma}$; $G_{\tau}=(1)$ for both the examples.
\item For the local homomorphisms we shall use the notation  $\phi_{ij}: G_{e_i}\map G_{v_j}$.
\end{enumerate}


\begin{figure}[h]
	\centering
	\begin{tikzpicture}
		\tikzset{vertex/.style = {shape=circle,draw,minimum size=2em}}
		\tikzset{edge/.style = {->,> = latex'}}
		% Vertices
		\node (v) at (0,0) {$v_1$};
		\node (u) at (3,-3) {$v_2$};
		\node (w) at (-3,-3) {$v_3$};
		\node (s) at (0,-1.9) {$\tau$};
		% Edges
		\draw[ ultra thick] (v) to node[midway,above,sloped] {$e_3$} (u) ;
		\draw[ ultra thick] (u) to node[midway,below,sloped] {$e_1$} (w);
		\draw[ ultra thick] (v) to node[midway,above,sloped] {$e_2$} (w);		
	\end{tikzpicture}
	\caption{}
	\label{pic 4}
\end{figure}

\begin{comment}

\begin{example}
	Let $Y$ be a triangle with vertices $v_1,v_2,v_3$, edges $e_1,e_2,e_3$ and let $\tau$ be the face of $Y$, see figure \ref{pic 4}. Suppose $G_{v_1}=\langle a,b|ab=ba\rangle, G_{v_2}=\langle c,d|cd=dc\rangle, G_{v_3}=\langle e,f|ef=fe\rangle$. Suppose all the edge groups $G_{e_1},G_{e_2},G_{e_3}$ are cyclic and the images of monomorphisms from $G_{e_3}$ to $G_{v_1},G_{v_2}$ are $\langle a\rangle$,$\langle c\rangle$ respectively. Similarly, images of monomorphisms for $e_2$ are $\langle e\rangle,\langle b\rangle$ and for $e_1$ are $\langle d\rangle,\langle f\rangle$. Since the face group $G_{\tau}$ is a subgroup of the intersection of edge groups, $G_{\tau}$ is trivial. Note that $\pi_1(\GG,Y)=\langle a,b,d|ab=ba,ad=da,bd=db\rangle$. Let $Y_1=e_3$. Then, $\pi_1(\GG,Y_1)=\langle a,b,d|ab=ba,ad=da\rangle$. Clearly, the natural map $\pi_1(\GG,Y_1)\rightarrow \pi_1(\GG,Y)$ is not injective.
\end{example}
\end{comment}


\begin{example}\label{not proper embedding}
\begin{enumerate}
\item Let $$G_{v_1}=\langle a,b|a^2,b^2\rangle, G_{v_2}=\langle c,d|c^2,d^2\rangle, G_{v_3} =\langle x,y,z|x^2,y^2,z^2\rangle.$$ 
\item Let $$G_{e_i}=\langle t_i| t_i^2\rangle, i=1,2,3.$$ 
The local homomorphisms are defined as follows.
	
\item  $\phi_{31}:G_{e_3}\map G_{v_1}$, $t_3\mapsto a$;  $\phi_{32}:G_{e_3}\map G_{v_2}$, $t_3\mapsto c$.
\item $\phi_{12}:G_{e_1}\map G_{v_2}$, $t_1\mapsto d$; $\phi_{13}:G_{e_1}\map G_{v_3}$, $t_1\mapsto y$.
\item $\phi_{21}:G_{e_2}\map G_{v_1}$, $t_2\map b$; $\phi_{23}:G_{e_2}\map G_{v_3}$, $t_2\mapsto x$.
\end{enumerate}  
Note that $(\GG,\YY)$ is developable, $G=\pi_1(\GG,\YY)=\langle a,b,d,z|a^2,b^2,d^2,z^2\rangle$ is hyperbolic and that
$G_{v_i}$'s are all quasiconvex in $\pi_1(\GG,\YY)$. Thus, the universal cover $B$ of $(\GG,\YY)$ is 
a hyperbolic space by Proposition \ref{mj-dahmani}. Let $\YY_1=e_3$ and let $(\GG,\YY_1)$ be the restriction of $(\GG,\YY)$ to $\YY_1$. 
Then $\pi_1(\GG,\YY_1)=G_{v_1} *_{G_{e_3}} G_{v_2}$ is quasiconvex in $\pi_1(\GG,\YY)$. The universal cover $B_1$ of 
$(\GG,\YY_1)$ is the Bass-Serre tree of $\pi_1(\GG,\YY_1)$. Consider the two vertices $v=G_{v_1}$ and $w_n=dbdb...db$ $(n-times)G_{v_2}$ 
of $B_1$. Note that $d_{B_1}(v,w_n)=n+1$. On the other hand, by construction of $B$ \textup{\cite[Theorem 2.13,III.C]{bridson-haefliger}}, one sees that $d_B(v,w_n)=2$. Hence, the natural map $B_1\rightarrow B$ is not a proper embedding and clearly there is no Cannon-Thurston map 
for the inclusion $B_1\map B$.
\end{example}
%It is worth noting that, in the above example, we can also use Proposition \ref{main converse} to show that there is no CT map from $B_1$ to $B$. 

The next example shows that the conclusion of Theorem \ref{edge qc} is false for a triangle of groups. For the definition of hyperbolic automorphism of a free group, one is referred to \cite{BF}.


\begin{example}\label{not qc edge}
\begin{enumerate}
\item Suppose $\mathbb F=\langle x,y,z\rangle$ is a free group on $3$ generators and $\phi$ is a hyperbolic automorphism 
(see \cite{BF}) of $\mathbb F$.
Let $G_{v_1}$ be the semidirect product $\mathbb Z \ltimes \mathbb F$ where we use $t$ to denote a generator of $\mathbb Z$, so that 
$$G_{v_1}=\langle x,y,z,t| twt^{-1}=\phi(w), w=x,y,z\rangle.$$ We note that $G_{v_1}$ is a hyperbolic group by the main result of \cite{BF}.
	
\item Suppose $$G_{v_3}=\langle a,b,c\rangle, G_{v_2}=\langle d,e\rangle$$ are free groups of rank $3$ and $2$ respectively.

\item Suppose $$G_{e_i}=\langle t_i \rangle, i=1,  3$$ are infinite cyclic. 
\item Suppose $$G_{e_2}=\langle u_1,u_2 \rangle $$ is a free group on two generators.
\item Suppose the local homomorphisms are defined as follows:
$$\phi_{21}: G_{e_2}\map G_{v_1}, u_1\mapsto a,u_2\mapsto b;$$
$$ \phi_{23}: G_{e_2}\map G_{v3}, u_1\mapsto z, u_2\mapsto x;$$
$$\phi_{12}:G_{e_1}\map G_{v_2}, t_1\mapsto c; \phi_{13}: G_{e_1}\map G_{v_3}, t_1\mapsto d;$$
$$\phi_{31}:G_{e_3}\map G_{v_1}, t_3\mapsto e; \phi_{32}:G_{e_3}\map G_{v_2}, t_3\mapsto y.$$
\end{enumerate}    
We note that $\pi_1(\GG,\YY)$ can be naturally identified with $G_{v_1}\ast \mathbb Z$. 
Let $\YY_1=e_1$ and let $(\GG,\YY_1)$ be the restriction of $(\GG,\YY)$. 
Then $\pi_1(\GG,\YY_1)=\mathbb F\ast \mathbb Z$ where $\mathbb F$ is the normal free subgroup of $G_{v_1}$ of rank $3$.
Clearly, $\pi_1(\GG,\YY_1)$ is not a quasiconvex subgroup of $\pi_1(\GG,\YY)$.
\end{example}
\begin{comment}
	
Next, we give an example of a developable triangle of groups such that the universal cover is not a CAT(0) space.
\begin{example}
	Let $Y$ be a Euclidean equilateral triangle as in figure \ref{pic 4}. Define a triangle of groups $(\GG,Y)$ in the following way:
	
	Assume that $G_{v_1}=\langle a,b,g|a^2,b^2,g^2,ab=ba,ag=ga,bg=gb\rangle$, $G_{v_2}=\langle c,d|c^2,d^2\\,cd=dc\rangle$, $G_{v_3} =\langle e,f,h|e^2,f^2,h^2,ef=fe,eh=he,fh=hf\rangle$. Assume that all the edge groups are of order $2$. Let the images of monomorphisms from $G_{e_3}$ to $G_{v_1},G_{v_2}$ be $\langle a \rangle,\langle c \rangle$. Similarly, images of monomorphisms for edge $e_1$ are $\langle d\rangle,\langle f\rangle$ and for $e_2$ are $\langle e\rangle,\langle b\rangle$. The face group $G_{\tau}$ is trivial. Note that Gersten-Stallings's angle \cite{gerstein-stalling} at each vertex is $\dfrac{\pi}{2}$. Thus, this triangle of groups is not non-positively curved in the sense of Gersten-Stallings \cite{gerstein-stalling}. Now, the universal cover $B$ of $(\GG,Y)$ is a $M_{\kappa}^2$ complex for $\kappa= 0$. By our choice of local groups, we have an injective loop of length $4$ in the link of a vertex of $B$ . Thus, the development does not satisfy the link condition by \cite[Lemma 5.6, II.5]{bridson-haefliger}. Hence, the development is not a CAT(0) space.
\end{example}
\end{comment}






